Video Game Level Repair via Mixed Integer Linear Programming

Recent advancements in procedural content generation via machine learning enable the generation of video-game levels that are aesthetically similar to human-authored examples. However, the generated levels are often unplayable without additional editing. We propose a generate-then-repair framework for automatic generation of playable levels adhering to specific styles. The framework constructs levels using a generative adversarial network (GAN) trained with human-authored examples and repairs them using a mixed-integer linear program (MIP) with playability constraints. A key component of the framework is computing minimum cost edits between the GAN generated level and the solution of the MIP solver, which we cast as a minimum cost network flow problem. Results show that the proposed framework generates a diverse range of playable levels, that capture the spatial relationships between objects exhibited in the human-authored levels.

==> amy-motivation-notes.tex <==



* Human-like is too vague: What makes these levels human-like?
--> -----

While the designers of systems that procedurally generate content may have different goals, in todo-based PCG the desire is often to capture the essence of  

* We focus on the problem of automatically generating human-like video game levels that are guaranteed to satisfy playability constraints.

-->

This first sentence assumes....
Note that playability with ML methods is the challenge and that playability with constraint-based techniques (and others) is guaranteed.
Constructive Methods ->  

We focus on the problem of automatically generating human-like video game levels that are guaranteed to satisfy playability constraints. For example, we would like to generate a variety of different Zelda levels; on one hand, we require these levels to be playable; for instance, they should include a character that the user can control, a door to exit the level and a key to open a door. At the same time, the levels should be diverse and human-like; a level with a character, a key and a door in adjacent tiles satisfies all playability requirements, but it does not have the appeal of a level created by a human designer. 

==> figures/average_path_cost.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.6\linewidth]{figs/average_cost_analysis.pdf}
%\includegraphics[width=0.49\linewidth]{figs/average_cost_analysis_finish_level.pdf}
\caption{The distribution of the length of the minimum path from the key to the door.}
\label{fig:average_path_cost}
\end{figure}

==> figures/edit_distance.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.8\linewidth]{figs/average_edit_distance_analysis.pdf}

\caption{The distribution of the average edit distance between levels from the same set.}
\label{fig:edit_distance}
\end{figure}

==> figures/kl_divergence.tex <==
\begin{table*}\centering
\ra{1.3}
\begin{tabular}{@{}rrrrcrrrcrrr@{}}\toprule
Model & Playable levels & Duplicated levels & Playable and unique levels \\ \midrule
Baseline GAN & 14.46\% & 63.16\% & 5.32\% \\
Baseline MILP & 100\% & 99\% &  1\%\\
CESAGAN~\citep{torrado:arxiv19} & 58\% & 37.6\% &  not reported\\
GAN + MILP (two-stage) & 100\% & 13.72\% & 86.27\% \\
%GAN + MILP (end-to-end) &  & & \\
\bottomrule
\end{tabular}
\caption{The encoding and visualization for the tiles in Zelda. Each symbol is encoded as a one-hot encoding for the GAN.}
\label{fig:compare_baseline}
\end{table*}

==> figures/visual_gan_generated.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.32\linewidth]{figs/gan_generated/14997.png}\includegraphics[width=0.32\linewidth]{figs/gan_generated/14913.png}
\includegraphics[width=0.32\linewidth]{figs/gan_generated/14913.png}
\caption{Example of DCGAN generated levels. Above are two unplayable levels and below are two playable levels.}
\label{fig:gan_generated}
\end{figure}

==> figures/visual_generated_two_stages.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.2\linewidth]{figs/two_stage_generated/0.png}\includegraphics[width=0.2\linewidth]{figs/two_stage_generated/21.png} \\ \includegraphics[width=0.2\linewidth]{figs/two_stage_generated/24.png}\includegraphics[width=0.2\linewidth]{figs/two_stage_generated/8.png}

\caption{Example of two-stage approach generated levels. All generated levels are playable.}
\label{fig:two_stage_generated}
\end{figure}

==> figures/visual_human_generated.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.2\linewidth]{figs/human_generated/0.png}\includegraphics[width=0.2\linewidth]{figs/human_generated/1.png}\includegraphics[width=0.2\linewidth]{figs/human_generated/2.png}\includegraphics[width=0.2\linewidth]{figs/human_generated/3.png}\includegraphics[width=0.2\linewidth]{figs/human_generated/4.png}

\caption{Example of human generated levels used for training.}
\label{fig:human_designed}
\end{figure}
